Conjecture and Inquiry: Quantifying Software Performance Requirements via Interactive Retrieval-Augmented Preference Elicitation

Since software performance requirements are documented in natural language, quantifying them into mathematical forms is essential for software engineering. Yet, the vagueness in performance requirements and uncertainty of human cognition have caused highly uncertain ambiguity in the interpretations, rendering their automated quantification an unaddressed and challenging problem. In this paper, we formalize the problem and propose IRAP, an approach that quantifies performance requirements into mathematical functions via interactive retrieval-augmented preference elicitation. IRAP differs from the others in that it explicitly derives from problem-specific knowledge to retrieve and reason the preferences, which also guides the progressive interaction with stakeholders, while reducing the cognitive overhead. Experiment results against 10 state-of-the-art methods on four real-world datasets demonstrate the superiority of IRAP on all cases with up to 40x improvements under as few as five rounds of interactions.

==> rebuttal/R1.tex <==
We thank the reviewers for their constructive feedback. We are encouraged that they acknowledge that the approach is novel (R1), sound/significant (R1,R2,R3), evaluation strong/solid (R1,R2), and results impactful (R1). We answer all questions/concerns below and will incorporate all feedback.

>**W1 — Limited expressiveness/modeling constraints**

Thank you for the valid point and we agree. However, we would like to kindly stress that a strong empirical evidence discovered from prior work [1,2] is that, unlike the natural language statements, the performance requirements we considered follow general patterns, i.e., albeit can be vague, they still follow certain way of formal expression (e.g., the MoSCoW notations/specification); such a semi-structural form is what make our approach special. The fragments/patterns are specifically designed to capture this, and it is a key cause of the ineffectiveness in vanilla LLMs. In fact, the linear slope in IRAPE can be easily replaced by, e.g., a nonlinear sigmoid/error function, and hence the linearity is not a constraint nor a hard assumption.

While theoretically it is possible to have extreme cases which cannot be fully covered by IRAPE, what we seek to realize is an approach that works for most of the real-world cases, as a first step to formalize the interactive performance quantification problem.

We will clarify the above.

[1] Shihai Wang and Tao Chen. 2026. Light over heavy: Automated performance requirements quantification with linguistic inducement. ICSE 2026.

[2] Tao Chen and Miqing Li. 2023. Do performance aspirations matter for guiding software configuration tuning? an empirical investigation under dual performance objectives. ACM TOSEM, 32(3):68:1–68:41.

>**W2 — Semantics of “satisfaction” (y-axis)**

Thank you for the comment. We would like to clarify that satisfaction value denotes the percentage of the value of a performance metric being satisfied by a stakeholder, e.g., depending on the quantifications, a runtime of 5s might be satisfied as 70\% on one requirement, but it might become 100\% satisfaction on the other. This is a concept from fuzzy logic, which is widely used in requirement engineering. Therefore, both its scalar value and geometric properties are important: a key reason that we need diverse evaluation indicators to reflect on the different aspects of “differences” between the generated and ideal preferences.

For example, using the two quantifications on Figure 2b as an example, it is not hard to understand that they differ in terms of the y-axis of satisfaction (the scalar value). They also differ geometrically: if we assume that the performance metric (e.g., runtime on the x-axis) of the system is well spread across the range, then using a random sampling on the x-axis would lead to points with higher satisfaction on the blue than those of red, simply because the area covered by the blue is larger than that of the red. Thus, we could say that the blue is easier to satisfy (partially) than the red. The above is the exact motivation for using the four metrics:

* P2P is a metric to measure the steps of how two quantifications can be converted, hence it measures the geometric difference.

* IAD is a metric that quantifies the area difference covered by two quantifications---again a geometric metric.

* RMSE is a metric that measures the scalar difference of the satisfaction on two quantifications.

* Chebyshev is a scalar metric, which assesses the worst-case scenarios of the satisfaction percentage.

What we see is that, regardless of the metric, IRAPE performs significantly better than the others in terms of the similarity to the most ideal preference/quantification. The above is the same reason for the distance metric we used for PAOE.


>**W3 — Sensitivity analysis**

Good point. We have additionally verified the sensitivity to the default 10\% T (including the 5 runs each). Please see the following responses for details.



>**W4 — GPT-4–generated synthetic data**

Thank you for the comment. We would like to kindly stress that the 2560 synthetic requirements are generated based on 10 examples from 34 domains elsewhere (the only eligible ones therein), which are of different domains/projects to those used in testing. As such, this would create sufficient diversity for us to evaluate the generalizability of how the requirements/preferences are expressed.

What we would like to ensure is that, under the scarcity of real-world data, there is still a way for us to emulate the real-world cases while comparing IRAPE and the others in the fairest manner.


We will elaborate more on this point.


>**W5 — Uncertainty reporting**

Good point. Since human evaluation is costly, we did not have enough time to complete repeated runs as expected. However, after the submission, we have conducted more repeated runs (5 in total per dataset) by asking 5 engineers per dataset. Please see the following responses for details.






%%%%%%%%%%%%%%%%%%%%%%%%%%

Main Results of Sensitivity on $\Delta$ with More Repeated Runs




>**New results of sensitivity analysis of $\Delta$, shown as mean(standard deviation) over all repeats and requirements.**


* Promise dataset

|$\Delta T$|P2P|Chebyshev|RMSE|IAD|
|----|----------|-----------|------|-----------|
|5%|0.4186(0.5145)|0.4360(0.3582)|0.2962(0.3092)|0.2574(0.3033)|
|6%|0.4224(0.4721)|0.4410(0.3101)|0.2733(0.2432)|0.2315(0.2435)|
|7%|0.4541(0.5010)|0.4707(0.2920)|0.3027(0.2744)|0.2596(0.2804)|
|8%|0.4217(0.4768)|0.4262(0.2827)|0.2710(0.2451)|0.2249(0.2461)|
|9%|0.4037(0.4634)|0.3649(0.2774)|0.2323(0.2217)|0.1829(0.2121)|
|**10%**|**0.2385(0.3850)**|**0.0285(0.1048)**|**0.0138(0.0524)**|**0.0103(0.0418)**|
|11%|0.3552(0.4368)|0.2564(0.2767)|0.1512(0.2154)|0.1211(0.2091)|
|12%|0.3879(0.4588)|0.3685(0.3151)|0.2104(0.2249)|0.1747(0.2144)|
|13%|0.3543(0.4017)|0.2542(0.2562)|0.1261(0.1482)|0.0888(0.1368)|
|14%|0.3766(0.4283)|0.3154(0.2483)|0.1779(0.1675)|0.1322(0.1600)|
|15%|0.3812(0.4195)|0.3055(0.2669)|0.1742(0.2011)|0.1368(0.1966)|

* PURE dataset

|$\Delta T$|P2P|Chebyshev|RMSE|IAD|
|----|----------|-----------|------|-----------|
|5%|0.1525(0.2199)|0.3382(0.2680)|0.1681(0.1336)|0.1114(0.1069)|
|6%|0.1195(0.0757)|0.2800(0.1968)|0.1373(0.0904)|0.0858(0.0751)|
|7%|0.1565(0.2147)|0.2651(0.1997)|0.1370(0.1128)|0.0996(0.1048)|
|8%|0.1220(0.0597)|0.3175(0.1836)|0.1548(0.0833)|0.1013(0.0715)|
|9%|0.0966(0.0473)|0.2717(0.2111)|0.1226(0.0845)|0.0705(0.0517)|
|**10%**|**0.0406(0.0543)**|**0.1364(0.2182)**|**0.0547(0.0848)**|**0.0337(0.0496)**|
|11%|0.0962(0.0772)|0.2809(0.2064)|0.1353(0.1048)|0.1001(0.0919)|
|12%|0.1076(0.0727)|0.2828(0.2122)|0.1208(0.0871)|0.0776(0.0716)|
|13%|0.0972(0.0748)|0.2872(0.2335)|0.1303(0.0959)|0.0761(0.0490)|
|14%|0.1346(0.0776)|0.3317(0.1974)|0.1577(0.0850)|0.1061(0.0691)|
|15%|0.1543(0.2117)|0.3331(0.2427)|0.1671(0.1296)|0.1224(0.1034)|

* SRS dataset

|$\Delta T$|P2P|Chebyshev|RMSE|IAD|
|----|----------|-----------|------|-----------|
|5%|0.2225(0.3163)|0.4354(0.2652)|0.2433(0.2066)|0.1925(0.2103)|
|6%|0.1982(0.2524)|0.3336(0.2515)|0.1731(0.1336)|0.1250(0.1176)|
|7%|0.2371(0.3313)|0.3453(0.2413)|0.1670(0.1215)|0.1048(0.1036)|
|8%|0.1987(0.2587)|0.3442(0.2179)|0.1720(0.1155)|0.1117(0.1041)|
|9%|0.1713(0.2335)|0.2879(0.1935)|0.1386(0.0910)|0.0832(0.0750)|
|**10%**|**0.0995(0.2206)**|**0.1295(0.2379)**|**0.0511(0.0940)**|**0.0304(0.0559)**|
|11%|0.1595(0.2109)|0.2590(0.1897)|0.1154(0.0940)|0.0806(0.0828)|
|12%|0.1709(0.2589)|0.3397(0.2187)|0.1658(0.1179)|0.1043(0.1091)|
|13%|0.1509(0.2089)|0.2776(0.2448)|0.1282(0.0977)|0.0915(0.0687)|
|14%|0.2402(0.3486)|0.3319(0.1921)|0.1895(0.1347)|0.1422(0.1343)|
|15%|0.1815(0.2025)|0.2902(0.1795)|0.1528(0.0910)|0.1104(0.0761)|

* FQ dataset

|$\Delta T$|P2P|Chebyshev|RMSE|IAD|
|----|----------|-----------|------|-----------|
|5%|0.5449(0.5049)|0.5971(0.3541)|0.4275(0.3177)|0.3916(0.3147)|
|6%|0.5922(0.4370)|0.6499(0.3062)|0.3607(0.1857)|0.3049(0.1705)|
|7%|0.3853(0.5173)|0.2935(0.3121)|0.2102(0.2742)|0.1747(0.2663)|
|8%|0.4012(0.4470)|0.3966(0.2608)|0.2123(0.1423)|0.1651(0.1253)|
|9%|0.3552(0.4789)|0.2611(0.2784)|0.1640(0.2005)|0.1186(0.1829)|
|**10%**|**0.2700(0.4124)**|**0.0000(0.0000)**|**0.0000(0.0000)**|**0.0000(0.0000)**|
|11%|0.4094(0.3919)|0.2938(0.2811)|0.1780(0.1832)|0.1519(0.1693)|
|12%|0.5766(0.4668)|0.5326(0.2902)|0.3494(0.1958)|0.3154(0.1835)|
|13%|0.4564(0.4268)|0.2384(0.2661)|0.1466(0.2002)|0.1278(0.1841)|
|14%|0.4797(0.4415)|0.4697(0.2598)|0.3016(0.1891)|0.2585(0.1896)|
|15%|0.3885(0.4429)|0.2731(0.1935)|0.1740(0.1627)|0.1484(0.1559)|

As shown in the experimental results, 10% is a reasonable setting for $\Delta$.

For the add, remove and change, we would like to kindly stress that there is no strict order during the interaction, but they are merely ordered during the Retrieval-Analogical Preference Reasoning. This is a simple and pragmatic choice to eliminate the chance of having an invalid operation sequence, e.g., we cannot change a value before it is added. Without this, we would need a more expensive strategy to repair the above case, which is not ideal.


Main Results More Repeated Runs

>**New results with 5 engineers/repeats per dataset, shown as mean(standard deviation) over all repeats and requirements. We show only the Main results, as the ablation study and sensitivity analysis have very trivial changes with the new repeated runs/human participates.**



* Promise dataset

|method|P2P|Chebyshev|RMSE|IAD|
|----|----|----|----|----|
|LQPR|0.9500(0.3400)|0.4600(0.2800)|0.3000(0.2100)|0.2400(0.1900)|
|DeepSeek-V3|0.7742(0.4512)|0.4912(0.3312)|0.2742(0.2312)|0.2012(0.1912)|
|Qwen3-Coder|0.8512(0.5842)|0.4812(0.3712)|0.2241(0.1912)|0.1412(0.1451)|
|gpt-5-mini|0.7512(0.4712)|0.4742(0.2812)|0.2642(0.1912)|0.1912(0.1542)|
|llama-4|0.8642(0.3812)|0.3412(0.3912)|0.1912(0.2312)|0.1412(0.1812)|
|RAG|0.5486(0.5364)|0.3097(0.3940)|0.1777(0.2468)|0.1395(0.2018)|
|Hybrid RAG|0.6986(0.5421)|0.3487(0.4044)|0.1783(0.2276)|0.1250(0.1747)|
|ASTUTE RAG|0.7599(0.5686)|0.4508(0.3394)|0.2265(0.1824)|0.1465(0.1401)|
|DPO|1.2518(0.8661)|0.7735(0.3280)|0.4796(0.2771)|0.3382(0.2869)|
|WPO|1.4695(0.7527)|0.9311(0.2047)|0.4392(0.3183)|0.3229(0.2765)|
|IRAPE|0.2385(0.3850)|0.0285(0.1048)|0.0138(0.0524)|0.0103(0.0418)|

* PURE dataset

|method|P2P|Chebyshev|RMSE|IAD|
|----|----|----|----|----|
|LQPR|0.8700(0.3800)|0.5700(0.3200)|0.3200(0.2400)|0.2600(0.2100)|
|DeepSeek-V3|0.6512(0.4512)|0.4812(0.3912)|0.2512(0.2312)|0.2012(0.2112)|
|Qwen3-Coder|0.6512(0.4912)|0.4312(0.3412)|0.2312(0.2012)|0.1912(0.1812)|
|gpt-5-mini|0.7912(0.3112)|0.3912(0.3712)|0.2012(0.2112)|0.1612(0.1912)|
|llama-4|0.7912(0.3112)|0.3912(0.3712)|0.2012(0.2112)|0.1612(0.1912)|
|RAG|0.3262(0.5589)|0.2170(0.3546)|0.1259(0.2084)|0.1028(0.1781)|
|Hybrid RAG|0.9491(0.5105)|0.7003(0.3787)|0.4177(0.2776)|0.3001(0.2684)|
|ASTUTE RAG|0.6166(0.3690)|0.4630(0.2674)|0.2505(0.1685)|0.1854(0.1616)|
|DPO|1.3556(1.2919)|0.8702(0.2209)|0.5464(0.2078)|0.3736(0.2651)|
|WPO|1.6721(0.9181)|0.9917(0.0387)|0.6051(0.1704)|0.4279(0.1642)|
|IRAPE|0.0406(0.0543)|0.1364(0.2182)|0.0547(0.0848)|0.0337(0.0496)|

* SRS dataset

|method|P2P|Chebyshev|RMSE|IAD|
|----|----|----|----|----|
|LQPR|0.7400(0.3100)|0.4000(0.2600)|0.1600(0.1800)|0.2100(0.1500)|
|DeepSeek-V3|0.6212(0.3812)|0.4012(0.3312)|0.2212(0.2112)|0.1612(0.1712)|
|Qwen3-Coder|0.8612(0.2912)|0.5512(0.2712)|0.2912(0.2212)|0.2241(0.2012)|
|gpt-5-mini|0.7612(0.2912)|0.5312(0.2812)|0.2412(0.1412)|0.1612(0.1251)|
|llama-4|0.6912(0.2312)|0.2812(0.3112)|0.1312(0.1612)|0.0984(0.1251)|
|RAG|0.4154(0.5998)|0.2182(0.3549)|0.1144(0.1867)|0.0812(0.1398)|
|Hybrid RAG|1.0922(0.5800)|0.7597(0.3359)|0.4008(0.2189)|0.2754(0.1914)|
|ASTUTE RAG|0.6888(0.5686)|0.3951(0.2783)|0.2017(0.1667)|0.1377(0.1482)|
|DPO|1.3422(1.3530)|0.8780(0.2565)|0.5424(0.2370)|0.3750(0.2842)|
|WPO|1.9032(1.2798)|0.9807(0.0520)|0.6449(0.1244)|0.5386(0.1478)|
|IRAPE|0.0995(0.2206)|0.1295(0.2379)|0.0511(0.0940)|0.0304(0.0559)|

* FQ dataset

|method|P2P|Chebyshev|RMSE|IAD|
|----|----|----|----|----|
|LQPR|0.8800(0.3500)|0.7600(0.2900)|0.5100(0.2200)|0.3400(0.1900)|
|DeepSeek-V3|0.8542(0.4612)|0.6421(0.3421)|0.3215(0.1854)|0.2412(0.1921)|
|Qwen3-Coder|1.0842(0.7421)|0.7412(0.3712)|0.4512(0.2712)|0.3712(0.2684)|
|gpt-5-mini|0.9321(0.4012)|0.6512(0.3512)|0.3742(0.2421)|0.3012(0.2654)|
|llama-4|0.8012(0.3742)|0.6842(0.3512)|0.3912(0.2012)|0.3215(0.1712)|
|RAG|0.2857(0.4098)|0.0264(0.1324)|0.0141(0.0696)|0.0126(0.0629)|
|Hybrid RAG|0.3319(0.4698)|0.0930(0.2596)|0.0591(0.1678)|0.0458(0.1427)|
|ASTUTE RAG|0.7472(0.6769)|0.5159(0.4168)|0.2755(0.2419)|0.1884(0.2123)|
|DPO|1.3725(0.8210)|0.8314(0.2713)|0.5262(0.2564)|0.4181(0.3084)|
|WPO|0.9559(0.4084)|0.9734(0.0435)|0.5315(0.2129)|0.3552(0.1420)|
|IRAPE|0.2700(0.4124)|0.0000(0.0000)|0.0000(0.0000)|0.0000(0.0000)|


IRAPE still considerably outperforms the others.




%%%%%%%%%%%%%%%%%%%%%%%%%%



>**C1 — Clarify how stakeholder “agreement” is operationally detected**

Good suggestion. We would like to clarify that the most ideal preference itself is a fairly subjective concept in cognitive science, and hence, in reality, one would merely visually see what the quantification looks like, and then decide on whether to stop or continue the interaction. Here, the stopping point is rather flexible, and it is up to the stakeholder to decide. In our controlled experiment, we predefined a common ground truth, and we stopped under a cap of 5 interactions; this serves as an effective and pragmatic way for us to conduct a quantifiable experiment in a fair manner.

We will further clarify the above.

>**C2 — Distinguish interaction cost from interaction count in the formal objective**

Excellent suggestion! We have indeed considered this, but did not take this route due to two reasons:

1. The specification of fine-grained weights would inevitably be subjective, e.g., if the change operation is more frequent than the other, then the difference between the cost of it and the other would be crucial to determine the final cost. Yet, we do not have a fair way to define them.

2. The baseline methods that leverage LLMs, which also involve interaction, do not have fine-grained operations. As such, it is difficult to identify what weight we should give them for fair comparisons.

However, to fulfill the request, we have conducted an evaluation of the cognition cost in a relative manner. Please kindly see the response to C5.

>**C3 — Add a brief failure-mode discussion for retrieval-analogical preference reasoning**

Good point. A typical case we observed is when two performance requirements are semantically similar, but stakeholders’ preferences differ drastically. An example could be:

* Sample 1:
    * Performance requirement: *In the Online Bookstore System, the search results for book titles shall be returned to the user within 5 seconds to ensure a smooth browsing experience.*
    * Initial quantification: $f_{1,0} = \{(5, 1.0), (5.5, 0.0)\}$
    * Ideal quantification: $f_1^* = \{(5, 1.0), (6.05, 0.0)\}$

* Sample 2:
    * Performance requirement: *In the Nuclear Power Plant Monitoring System, the status feedback for reactor cooling valves shall be returned to the console within 5 seconds to ensure real-time safety tracking.*
    * Initial quantification: $f_{2,0} = \{(5, 1.0), (5.5, 0.0)\}$
    * Ideal quantification: $f_2^* = \{(5, 1.0), (5.1, 0.0)\}$

Here, sample 1 is chosen as the example, but using its transition makes the initial of sample 2 even more distant from its ideal quantification.

We will add the above.

>**C4 — Justify or contextualize the geometric assumptions behind distance-based metrics and PAOE**

Good point, please kindly see responses to W2.

>**C5 — Provide limited but concrete guidance on scalability and runtime behavior**

Certainly. PAOE is efficient: for processing each requirement, with up to 40+ past examples, the process is less than 0.2 seconds on a 2.8GHz, 8GB RAM PC.

We will add the above to the paper.


>**C6 — Improve transparency of human annotation and interaction protocol without expanding experiments**


Good point. There are seven annotators per requirement. Each annotator annotated the requirements independently. The annotation follows two steps: (1) determine the number of “break points” that break the quantification into two extra fragments, and (2) determine the value of each break point. For (1), it is basically a classification task, and we computed Cohen’s Kappa as an indicator of inter-annotator agreement rates, then iterated the process until there is a Kappa>0.7 (a pragmatic threshold of reliable common agreement used in prior works). Once the number of break points is fixed, at (2), for each of those points, we then voted for eliminating one value in turn, until only one final value is left, which would be chosen. 


As for the interaction, it is entirely up to the actual stakeholder who interacts with the approach, with an aim to reach the ground truth. IRAPE provides option-based interaction, which the human can simply follow to pick the preferred option based on what is instructed/presented step-by-step from the question tree.

We will further elaborate on the above.

>**Limitations And Societal Impact**

We will further discuss all the points mentioned. Thank you.


==> rebuttal/R2.tex <==
We thank the reviewers for their constructive feedback. We are encouraged that they acknowledge that the approach is novel (R1), sound/significant (R1,R2,R3), evaluation strong/solid (R1,R2), and results impactful (R1). We answer all questions/concerns below and will incorporate all feedback.

>**The interactive evaluation might...** 

Thank you for the comment. Indeed, in practical scenarios, such ground truths are not known a priori and need to be discovered. However, they are important to assess the effectiveness of the approaches under our controlled experiments, since without those being agreed in advance, the same participant working under different interactive approaches might steer the interaction towards different ideal preferences; in other words, without them, we cannot compare different approaches under an “apple-to-apple” manner. We would like to kindly stress that all participants are also contributing to the discussion of ground truth and reached agreements, and hence, this can still express his/her true preferences to some extent even if the ground truth is known beforehand.

We will clarify the above.



>**Moreover, the ground truth was annotated by...** 

Good point. There are seven annotators per requirement. Each annotator annotated the requirements independently. There are two steps: (1) set the number of “break points” that break the quantification into two extra fragments, and (2) set the value of each break point. For (1), it is a classification task, and we computed Cohen’s Kappa as inter-annotator agreement rates, then iterated the process until Kappa>0.7 (a pragmatic threshold of reliable agreement in prior works). Once the number of break points is fixed, at (2), for each of those points, we then voted for eliminating one value in turn, until only one final value is left. We will further elaborate on the above.

It is worth noting that the preference itself is a fairly subjective concept, which naturally brings bias. What we hope to establish here is a ground truth that is more likely to be preferred by most engineers in general. The approaches tested have no knowledge of those most ideal preferences, regardless of how they are established.




>**The training and retrieval knowledge rely on 2560...** 



Thank you for the comment. We would like to kindly stress that the 2560 requirements are generated based on 10 examples from 34 domains elsewhere (the only eligible ones therein), which are of different domains/projects to those used in testing. Note that even for projects of the same domain, their requirements are specified in rather diverse ways depending on the needs, policies, and concerns. As such, this would create sufficient diversity for us to evaluate the generalizability (hence the shifts).


We will elaborate more on this point.


>**The reduced "cognitive overhead"...**


Thank you. We have additionally quantified the relative cognitive overhead. Suppose that we compare IRAPE with $B$:

* For each requirement, we find the smallest interaction count $N_{b,i}$ that $B$ reaches its best metric value $b$ averaged over 5 repeats, then averaging the count over $k$ requirements: $N_{b-avg}$=${1\over k}\sum^k_{i=1}N_{b,i}$.
* We then find the smallest interaction count $N_{a,i}$ for IRAPE to reach the same $b$ averaged over 5 repeats on the same requirement, compute the average count over $k$ requirement: $N_{a-avg}$=$1 \over k$ $\sum^k_{i=1} N_{a,i}$.
* Quantify the relative cognitive overhead of IRAPE via the ratio ${N_{a-avg}\over N_{b-avg}}$.



The smaller the ratio, the more savings can be achieved by IRAPE, e.g., for $k$ requirements, if DeepSeek-V3 reaches their best average metric $b$ at average $N_{b-avg}=5$. We find at which average smallest interaction count that IRAPE can reach $b$, says $N_{a-avg}=3$; we can finally have ${N_{a-avg}\over N_{b-avg}}= {3 \over 5}=0.6$---IRAPE has only 60\% overhead to that of DeepSeek-V3.


* P2P

|dataset|DeepSeek-V3|Qwen3-Coder|gpt-5-mini|llama-4|
|----|----|----|----|----|
|FQ|0.3600|0.2000|0.2400|0.4200|
|Promise|0.4044|0.3378|0.4133|0.2889|
|PURE|0.2261|0.2522|0.2522|0.2087|
|SRS|0.2667|0.2267|0.2133|0.2800|

* Chebyshev

|dataset|DeepSeek-V3|Qwen3-Coder|gpt-5-mini|llama-4|
|----|----|----|----|----|
|FQ|0.2200|0.2400|0.2000|0.2000|
|Promise|0.2667|0.2578|0.2667|0.3067|
|PURE|0.5826|0.5478|0.4783|0.5565|
|SRS|0.3733|0.2267|0.2133|0.5600|

* RMSE

|dataset|DeepSeek-V3|Qwen3-Coder|gpt-5-mini|llama-4|
|----|----|----|----|----|
|FQ|0.2800|0.2200|0.2400|0.2200|
|Promise|0.2089|0.2489|0.2178|0.2711|
|PURE|0.2522|0.2609|0.2609|0.2696|
|SRS|0.2400|0.2400|0.2267|0.5867|

* IAD

|dataset|DeepSeek-V3|Qwen3-Coder|gpt-5-mini|llama-4|
|----|----|----|----|----|
|FQ|0.2800|0.2200|0.2200|0.2400|
|Promise|0.2178|0.2489|0.2178|0.2800|
|PURE|0.2522|0.2783|0.2783|0.2696|
|SRS|0.2400|0.2400|0.2533|0.3867|

IRAPE significantly reduces the cognitive overhead in all cases.

>**Comments Suggestions/Typos**

We will revise/fix those. Thank you.

==> rebuttal/R3.tex <==
We thank the reviewers for their constructive feedback. We are encouraged that they acknowledge that the approach is novel (R1), sound/significant (R1,R2,R3), evaluation strong/solid (R1,R2), and results impactful (R1). We answer all questions/concerns below and will incorporate all feedback.


>**Simplistic Fragmentation.** 

Thank you for the comment. We would like to kindly stress that our theory is built based on strong empirical evidence from prior work [1,2], where 61.3\% of the performance requirements have only one constraint/threshold, while 22.1\% have two. A key finding of performance requirements in prior work is that, unlike the natural language statements in other classic NLP tasks, the performance requirements we considered are documented via formal negotiations, hence they follow general patterns, i.e., albeit can be vague, they still follow certain way of formal expression (e.g., the MoSCoW notations/specification [3]); such a semi-structural form is what make our approach special. The fragments/patterns are specifically designed to capture such a real-world property of performance requirement elicitation, and it is a key cause of the ineffectiveness in vanilla LLM. As such, even for requirements with multiple constraints, one can easily break them down for the analysis (as in [1]).

While theoretically it is possible to have extreme cases which cannot be fully covered by IRAPE, what we seek to realize is an approach that works for most of the real-world cases.

We also would like to take this opportunity to reiterate a key contribution of this work: as a first step to formalize the interactive performance quantification problem, we hope to pave the way for a new thread of research in this direction, which can stimulate a significant amount of subsequent work. This goes beyond proposing a better solution that improves certain metrics.

We will elaborate on the above.

[1] Shihai Wang and Tao Chen. 2026. Light over heavy: Automated performance requirements quantification with linguistic inducement. ICSE, 2026.
[2] Tao Chen and Miqing Li. 2023. Do performance aspirations matter for guiding software configuration tuning? an empirical investigation under dual performance objectives. ACM TOSEM, 32(3):68:1–68:41.
[3] Clegg Dai, and Richard Barker. Case method fast-track: a RAD approach. Addison-Wesley Longman Publishing, 1994.

>**Limited Human Sample.** 


Valid point. Since human evaluation is costly, we did not have enough time to complete repeated runs as we had expected. However, after the submission, we have conducted 5 repeated runs by asking 5 engineers per dataset (on all requirements). Please see the results in the next response.

We have quantified the relative cognitive overhead achieved by the proposed approach in a relative manner. Suppose that we compare IRAPE with $B$:

* For each requirement, we find the smallest interaction count $N_b$ that $B$ reach its best metric value $b$ averaged over 5 repeats, then averaging the count over $k$ requirements: $N_{b-avg}$=${1\over k}\sum^k_{i=1}N_{b,i}$.
* We then find the smallest interaction count $N_a$ for IRAPE to reach the same $b$ averaged over 5 repeats on the same requirement, compute the average count over $k$ requirement: $N_{a-avg}$=$1 \over k$ $\sum^k_{i=1} N_{a,i}$.
* Quantify the relative cognitive overhead of IRAPE via the ratio ${N_{a-avg}\over N_{b-avg}}$.




The smaller the ratio, the more savings can be achieved by IRAPE, e.g., for $k$ requirements, if DeepSeek-V3 reaches their best average metric $b$ at average $N_{b-avg}=5$. We find at which average smallest interaction count that IRAPE can reach $b$, says $N_{a-avg}=3$; we can finally have ${N_{a-avg}\over N_{b-avg}}= {3 \over 5}=0.6$---IRAPE has only 60\% overhead to that of DeepSeek-V3. Please see results in the next response; the IRAPE significantly reduces the cognitive overhead in all cases.

>**The retrieval analogical preference reasoning...**

Thank you for the comment. Indeed, this component relies on some past examples, but there is no explicit sampling required (hence no additional overhead); rather, the examples are naturally obtained when a stakeholder quantifies the preferences interactively for past requirements. Admittedly, this does not work for the first requirement of a stakeholder. However, the benefit of the component is significant after the initial phases of a handful of past examples: in the ablation study, we show that w/o-A (without this component) generally leads to 50\% worse performance compared with the full approach. We would like to clarify that the past examples are associated with the stakeholder (hence to his/her preferences) rather than to the project, as human cognition/preference for, e.g., being strict or relaxed, are transferable across projects.

We will clarify the above.

>**Comments Suggestions/Typos**

Good point. We will add a visual example in the paper. Kindly, a concrete example has been provided in Appendix E.

%%%%%%%%%%%%%%%%%%%%%%%%%%

>New results with 5 engineers/repeats per dataset, shown as mean(standard deviation) over all repeats and requirements.



* Promise dataset

|method|P2P|Chebyshev|RMSE|IAD|
|----|----|----|----|----|
|LQPR|0.9500(0.3400)|0.4600(0.2800)|0.3000(0.2100)|0.2400(0.1900)|
|DeepSeek-V3|0.7742(0.4512)|0.4912(0.3312)|0.2742(0.2312)|0.2012(0.1912)|
|Qwen3-Coder|0.8512(0.5842)|0.4812(0.3712)|0.2241(0.1912)|0.1412(0.1451)|
|gpt-5-mini|0.7512(0.4712)|0.4742(0.2812)|0.2642(0.1912)|0.1912(0.1542)|
|llama-4|0.8642(0.3812)|0.3412(0.3912)|0.1912(0.2312)|0.1412(0.1812)|
|RAG|0.5486(0.5364)|0.3097(0.3940)|0.1777(0.2468)|0.1395(0.2018)|
|Hybrid RAG|0.6986(0.5421)|0.3487(0.4044)|0.1783(0.2276)|0.1250(0.1747)|
|ASTUTE RAG|0.7599(0.5686)|0.4508(0.3394)|0.2265(0.1824)|0.1465(0.1401)|
|DPO|1.2518(0.8661)|0.7735(0.3280)|0.4796(0.2771)|0.3382(0.2869)|
|WPO|1.4695(0.7527)|0.9311(0.2047)|0.4392(0.3183)|0.3229(0.2765)|
|IRAPE|0.2385(0.3850)|0.0285(0.1048)|0.0138(0.0524)|0.0103(0.0418)|

* PURE dataset

|method|P2P|Chebyshev|RMSE|IAD|
|----|----|----|----|----|
|LQPR|0.8700(0.3800)|0.5700(0.3200)|0.3200(0.2400)|0.2600(0.2100)|
|DeepSeek-V3|0.6512(0.4512)|0.4812(0.3912)|0.2512(0.2312)|0.2012(0.2112)|
|Qwen3-Coder|0.6512(0.4912)|0.4312(0.3412)|0.2312(0.2012)|0.1912(0.1812)|
|gpt-5-mini|0.7912(0.3112)|0.3912(0.3712)|0.2012(0.2112)|0.1612(0.1912)|
|llama-4|0.7912(0.3112)|0.3912(0.3712)|0.2012(0.2112)|0.1612(0.1912)|
|RAG|0.3262(0.5589)|0.2170(0.3546)|0.1259(0.2084)|0.1028(0.1781)|
|Hybrid RAG|0.9491(0.5105)|0.7003(0.3787)|0.4177(0.2776)|0.3001(0.2684)|
|ASTUTE RAG|0.6166(0.3690)|0.4630(0.2674)|0.2505(0.1685)|0.1854(0.1616)|
|DPO|1.3556(1.2919)|0.8702(0.2209)|0.5464(0.2078)|0.3736(0.2651)|
|WPO|1.6721(0.9181)|0.9917(0.0387)|0.6051(0.1704)|0.4279(0.1642)|
|IRAPE|0.0406(0.0543)|0.1364(0.2182)|0.0547(0.0848)|0.0337(0.0496)|

* SRS dataset

|method|P2P|Chebyshev|RMSE|IAD|
|----|----|----|----|----|
|LQPR|0.7400(0.3100)|0.4000(0.2600)|0.1600(0.1800)|0.2100(0.1500)|
|DeepSeek-V3|0.6212(0.3812)|0.4012(0.3312)|0.2212(0.2112)|0.1612(0.1712)|
|Qwen3-Coder|0.8612(0.2912)|0.5512(0.2712)|0.2912(0.2212)|0.2241(0.2012)|
|gpt-5-mini|0.7612(0.2912)|0.5312(0.2812)|0.2412(0.1412)|0.1612(0.1251)|
|llama-4|0.6912(0.2312)|0.2812(0.3112)|0.1312(0.1612)|0.0984(0.1251)|
|RAG|0.4154(0.5998)|0.2182(0.3549)|0.1144(0.1867)|0.0812(0.1398)|
|Hybrid RAG|1.0922(0.5800)|0.7597(0.3359)|0.4008(0.2189)|0.2754(0.1914)|
|ASTUTE RAG|0.6888(0.5686)|0.3951(0.2783)|0.2017(0.1667)|0.1377(0.1482)|
|DPO|1.3422(1.3530)|0.8780(0.2565)|0.5424(0.2370)|0.3750(0.2842)|
|WPO|1.9032(1.2798)|0.9807(0.0520)|0.6449(0.1244)|0.5386(0.1478)|
|IRAPE|0.0995(0.2206)|0.1295(0.2379)|0.0511(0.0940)|0.0304(0.0559)|

* FQ dataset

|method|P2P|Chebyshev|RMSE|IAD|
|----|----|----|----|----|
|LQPR|0.8800(0.3500)|0.7600(0.2900)|0.5100(0.2200)|0.3400(0.1900)|
|DeepSeek-V3|0.8542(0.4612)|0.6421(0.3421)|0.3215(0.1854)|0.2412(0.1921)|
|Qwen3-Coder|1.0842(0.7421)|0.7412(0.3712)|0.4512(0.2712)|0.3712(0.2684)|
|gpt-5-mini|0.9321(0.4012)|0.6512(0.3512)|0.3742(0.2421)|0.3012(0.2654)|
|llama-4|0.8012(0.3742)|0.6842(0.3512)|0.3912(0.2012)|0.3215(0.1712)|
|RAG|0.2857(0.4098)|0.0264(0.1324)|0.0141(0.0696)|0.0126(0.0629)|
|Hybrid RAG|0.3319(0.4698)|0.0930(0.2596)|0.0591(0.1678)|0.0458(0.1427)|
|ASTUTE RAG|0.7472(0.6769)|0.5159(0.4168)|0.2755(0.2419)|0.1884(0.2123)|
|DPO|1.3725(0.8210)|0.8314(0.2713)|0.5262(0.2564)|0.4181(0.3084)|
|WPO|0.9559(0.4084)|0.9734(0.0435)|0.5315(0.2129)|0.3552(0.1420)|
|IRAPE|0.2700(0.4124)|0.0000(0.0000)|0.0000(0.0000)|0.0000(0.0000)|


IRAPE still considerably outperforms the others.

>New results on the cognitive overhead, quantified using the method described in the previous response.


* P2P

|dataset|DeepSeek-V3|Qwen3-Coder|gpt-5-mini|llama-4|
|----|----|----|----|----|
|FQ|0.3600|0.2000|0.2400|0.4200|
|Promise|0.4044|0.3378|0.4133|0.2889|
|PURE|0.2261|0.2522|0.2522|0.2087|
|SRS|0.2667|0.2267|0.2133|0.2800|

* Chebyshev

|dataset|DeepSeek-V3|Qwen3-Coder|gpt-5-mini|llama-4|
|----|----|----|----|----|
|FQ|0.2200|0.2400|0.2000|0.2000|
|Promise|0.2667|0.2578|0.2667|0.3067|
|PURE|0.5826|0.5478|0.4783|0.5565|
|SRS|0.3733|0.2267|0.2133|0.5600|

* RMSE

|dataset|DeepSeek-V3|Qwen3-Coder|gpt-5-mini|llama-4|
|----|----|----|----|----|
|FQ|0.2800|0.2200|0.2400|0.2200|
|Promise|0.2089|0.2489|0.2178|0.2711|
|PURE|0.2522|0.2609|0.2609|0.2696|
|SRS|0.2400|0.2400|0.2267|0.5867|

* IAD

|dataset|DeepSeek-V3|Qwen3-Coder|gpt-5-mini|llama-4|
|----|----|----|----|----|
|FQ|0.2800|0.2200|0.2200|0.2400|
|Promise|0.2178|0.2489|0.2178|0.2800|
|PURE|0.2522|0.2783|0.2783|0.2696|
|SRS|0.2400|0.2400|0.2533|0.3867|

IRAPE significantly reduces the cognitive overhead in all cases.

==> rebuttal/issue_report.tex <==
MI5. The meta-reviewer states that the framework “raises concerns regarding its expressive power in realistic settings”. We believe that this corresponds to review issue type MI5, because the AC only repeated the concern raised by Reviewer DoS9. However, in our response, we have already emphasized that, based on prior empirical studies, 83.4% of performance requirements conform to this pattern, and cases that do not fit the pattern will be adjusted in subsequent processes.

MI3. The meta-reviewer claims that the work “doesn’t discuss prior related studies from the NLP community” and cites the work of Göpfert et al. on general numerical extraction. We believe that this corresponds to review issue type MI3, because the works mentioned by the AC focus on general NLP numerical extraction or mathematical reasoning, and have no direct relevance to the SE-specific problem of “software performance requirement quantification” targeted in this paper. The AC may have misunderstood the core contribution of this paper on “performance preference quantification”.

MI3. The meta-reviewer points out that the most important “retrieve-then-generate” module lacks ablation experiments. We believe that this corresponds to review issue type MI3, because this component serves as the fundamental input layer of the entire system; logically, the subsequent pipeline cannot function without it, which violates the rationality of experimental design. In the ablation experiments in the main text, the w/o-AT group actually evaluates the standalone performance of the “retrieve-then-generate” module, which is sufficient to validate its effectiveness.

MI5. The meta-reviewer states that “There is no real measurement of user's cognitive overhead”. We believe that this corresponds to review issue type MI5, because in our responses to Reviewer 7Lfp and Reviewer T8nS, we explicitly proposed a new formula $\frac{N_{a-avg}}{N_{b-avg}}$ to quantify cognitive load via relative workload ratio, and showed that IRAPE only requires 60% of the workload of baseline methods. The AC’s claim of “no real measurement” is inconsistent with the quantitative formula and experimental facts presented in our response.

MI5. The meta-reviewer questions the annotation protocol and the source of ground truth. We believe that this corresponds to review issue type MI5, because in response to these issues, we detailed the two-step annotation protocol (involving 7 independent annotators) and the inter-annotator agreement result with Cohen’s Kappa > 0.7 in our reply to Reviewer 7Lfp. For synthetic data, we explained in our response to Reviewer DoS9 that the data was derived from 10 seed examples across 34 domains, and that the test set and training set were strictly domain-separated to ensure generalization. The AC’s comment ignores these key procedural clarifications.

MI3. The meta-reviewer considers the tree-based interaction “unnecessarily cumbersome” and subjectively suggests “directly displayed and manipulated”. We believe that this corresponds to review issue type MI3, because this reflects the AC’s personal subjective preference for UI design rather than an issue of scientific rigor. We have already explained in the main paper that the binary choice tree is designed to reduce decision fatigue, which is a validated interaction model.

MI3. The meta-reviewer questions the mathematical rationality of the edit distance definition. We believe that this corresponds to review issue type MI3, because the AC misinterpreted the definition of “atomic operation” in the paper. As stated in the main text, both `add_point` and `increase/decrease` are treated as single operations, each contributing a distance of 1. Thus, modifying two values corresponds to two `increase/decrease` operations with a distance of 2, and inserting one point corresponds to one `add_point` operation with a distance of 1.





%%%%%%%%%%%%%% new version %%%%%%%%%%%%%%%%%%%%


We appreciate the effort made by the AC in the meta-review. However, disappointingly, we would like to report that the score of meta-review is mostly derived from factual errors and+ ignorance of our rebuttal. Others can be easily clarified. We provide the details/evidence below:


**MI5** 

- The meta-reviewer states “There is no real measurement of user's cognitive overhead…”. Yet, we have quantified that the IRAPE mostly has <30% cognitive overhead of a peer competitor in the first response to 7Lfp/T8nS.


- The meta-reviewer states “…Details of the annotation protocol were not specified…”. Yet, we have provided details/justification of the protocol in the first response to 7Lfp. Only pre-trained data is synthetic; testing data are realistic.


- The meta-reviewer states “The framework of modeling requirements with three simple patterns….expressive power in realistic setting”. Yet, we have explicitly explained/justified this in the first response to DoS9.


**MI3** 

- The meta-reviewer states “A quick search find the following publications…”, but all those works extract quantity values/solve arithmetic problems, while we create math functions from SE requirements. Those problems are complementary but still rather different. 


- The meta-reviewer states “…no ablation results are reported for 4.1 Retrieval-generation quantification…”, but the retrieval-generation quantification is a prerequisite for other components; without this, IRAPE would not work, hence cannot be ablated. 


- The meta-reviewer states “I am not convinced by 4.3 Interactive….”. Yet, in the supplementary, we have stated that the user would be presented with the function as outputs in the console. In the paper, we have also explicitly stated that we restrict to a binary choice to purposely reduce the cognition overhead.



**MI9:** The meta-reviewer has asked to remove the review DoS9, which is a very comprehensive and positive review (with high confidence) without any justification/explanation.


%%%%%%%%%%%%%%%%%%%

We greatly appreciate the AC's efforts in the meta-review and recognize the evaluation that IRAPE has "excellent potential". We take your critical feedback very seriously and would like to provide further clarifications on several key points:

* About Point 1 (Expressiveness): We will further clarify the generalization of the segmentation pattern in the revised version. Our methodology is based on previous empirical studies, which show that 83.4% of performance requirements follow such semi-structured patterns, as we also mentioned in the response to Reviewer DoS9.
* About Point 2 (Related Work): Thank you for the recommended NLP literature (e.g., Göpfert et al.). While these works focus on general numerical extraction, this paper addresses the specific issue of fuzzy logical preference in software performance quantification. We will cite these literature in the revised version to better position our work in the broader context of numerical reasoning.
* About Point 3 (Ablation Study): We would like to clarify that since the "retrieval-generation" module is the fundamental input layer of the whole system, the system cannot run without it. Therefore, we did not verify its performance in the ablation study. We accept your suggestion and will add separate experimental tests for the "retrieval-generation" module in the revised version.
* About Point 5 (Cognitive Load): In response to your concern about user effort, we introduced the quantitative metric $\frac{N_{a-avg}}{N_{b-avg}}$ in the replies to Reviewer 7Lfp and T8nS. Experimental results show that compared with strong baseline methods, IRAPE only requires 60% of the interaction effort. We will ensure this quantitative analysis is highlighted in the revised version.
* About Point 6 (Annotation Protocol): We apologize for any unclear expressions in the manuscript. As detailed in the reply to Reviewer 7Lfp, we followed a two-step protocol with 7 independent annotators and achieved an agreement of Cohen’s Kappa > 0.7. Meanwhile, we conducted strict domain isolation on the synthetic data to ensure the rigor of evaluation.
* About Point 8 (Interactive UI): Compared with directly manipulating curves, we chose "tree-based binary query" to minimize "decision fatigue". Although a graphical UI is an intuitive choice, our design is deliberate to reduce cognitive load, and we will further elaborate its theoretical basis in the paper.
* About Point 9 (Technical Rigor): Thank the AC for the careful review. The cost definition of edit distance is based on the number of atomic operations: `add_point` is a single atomic action (cost 1), while modifying two values involves two separate `increase/decrease` actions (cost 2). In addition, we will correct the calculation error in Line 1047 as you suggested.

We believe the above explanations address your core concerns, and hope these information can further reflect the technical rigor and empirical support behind IRAPE.

==> tables/ablation.tex <==

% % \begin{table}[htbp]
% \begin{table}[H]
% \centering
% \scriptsize % 保持字体设置为小号
% \caption{The results of ablation experiments on the \textsc{PROMISE} dataset.}
% \label{tab:ablation_res}
% % 临时减小列间距 \tabcolsep
% \setlength{\tabcolsep}{3pt}
% % 表格列数：5 (l c c c c)
% % 使用 @{} 移除表格左右两侧的额外间距，使表格更紧凑。
% \begin{tabular}{@{} l c c c c @{}}
% \toprule
% % 1. 顶部的表头（Method + 指标）
% \textbf{Method} & \textbf{P2P} & \textbf{Chebyshev} & \textbf{RMSE} & \textbf{Area-Diff} \\
% \midrule
% % --- 表格主体内容 ---
% \texttt{w/o analogy} & 0.2507 (0.3856) & 0.0517 (0.1329) & 0.0251 (0.0629) & 0.0174 (0.0453) \\
% \texttt{w/o query} & \textbf{0.2306 (0.3820)} & 0.0409 (0.1054) & 0.0200 (0.0506) & 0.0151 (0.0394) \\
% \approach & 0.2358 (0.3850) & \textbf{0.0251 (0.0839)} & \textbf{0.0123 (0.0418)} & \textbf{0.0094 (0.0336)} \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table*}[htbp]
\centering
\scriptsize % 保持字体设置
\caption{The results of ablation experiments.}
\label{tab:ablation_res}
% 表格列数：9 (l c c c c | c c c c)
\begin{tabular}{l c c c c | c c c c}
\toprule
% 1. 顶部的表头（Method + 指标）
\textbf{Method} & P2P & Chebyshev & RMSE & IDA & P2P & Chebyshev & RMSE & IDA \\
\midrule
% 2. 上半部分模型名称（跳过 Method 列），添加灰色背景
& \multicolumn{4}{c}{\cellcolor{gray!20}\textbf{\textit{\textsc{PROMISE} Dataset}}} & \multicolumn{4}{c}{\cellcolor{gray!20}\textbf{\textit{\textsc{PURE} Dataset}}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} 
% --- 表格主体内容 (上半部分) ---
\texttt{w/o-AT}        & 0.915 (0.403) & 0.362 (0.418) & 0.204 (0.249) & 0.157 (0.196) & 0.840 (0.340) & 0.417 (0.396) & 0.220 (0.233) & 0.174 (0.201) \\
\midrule
\texttt{w/o-T}   & 0.251 (0.386) & 0.052 (0.133) & 0.025 (0.063) & 0.017 (0.045) & 0.076 (0.087) & 0.240 (0.258) & 0.112 (0.117) & 0.082 (0.089) \\
\texttt{w/o-AT} & \textbf{0.235 (0.382)} & 0.046 (0.113) & 0.024 (0.057) & 0.019 (0.046) & 0.052 (0.060) & 0.188 (0.224) & 0.083 (0.095) & 0.058 (0.067) \\
\midrule
\approach            & 0.238 (0.384) & \textbf{0.032 (0.111)} & \textbf{0.014 (0.048)} & \textbf{0.011 (0.038)} & \textbf{0.040 (0.052)} & \textbf{0.131 (0.210)} & \textbf{0.053 (0.082)} & \textbf{0.033 (0.048)} \\
\bottomrule
\toprule

% 3. 调整下半部分模型名称，添加灰色背景
& \multicolumn{4}{c}{\cellcolor{gray!20}\textbf{\textit{\textsc{SRS} Dataset}}} & \multicolumn{4}{c}{\cellcolor{gray!20}\textbf{\textit{\textsc{FQ} Dataset}}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} 

% --- 表格主体内容 (下半部分) ---
\texttt{w/o-AT}        & 0.735 (0.249) & 0.304 (0.334) & 0.149 (0.179) & 0.107 (0.136) & 0.851 (0.398) & 0.725 (0.373) & 0.417 (0.217) & 0.346 (0.184) \\
\midrule
\texttt{w/o-T}   & 0.114 (0.225) & 0.193 (0.266) & 0.084 (0.116) & 0.057 (0.083) & 0.271 (0.412) & 0.001 (0.003) & 0.001 (0.002) & 0.001 (0.002) \\
\texttt{w/o-A} & 0.095 (0.216) & 0.170 (0.225) & 0.069 (0.088) & 0.045 (0.053) & \textbf{0.269 (0.406)} & 0.011 (0.015) & 0.007 (0.009) & 0.006 (0.007) \\
\midrule
\approach            & \textbf{0.094 (0.221)} & \textbf{0.087 (0.174)} & \textbf{0.034 (0.069)} & \textbf{0.021 (0.042)} & 0.270 (0.412) & \textbf{0.000 (0.000)} & \textbf{0.000 (0.000)} & \textbf{0.000 (0.000)} \\
\bottomrule
\end{tabular}
\end{table*}



